Ambisonics Binaural Rendering via Masked Magnitude Least Squares

Ambisonics rendering has become an integral part of 3D audio for headphones. It works well with existing recording hardware, the processing cost is mostly independent of the number of sound sources, and it elegantly allows for rotating the scene and listener. One challenge in Ambisonics headphone rendering is to find a perceptually well behaved low-order representation of the Head-Related Transfer Functions (HRTFs) that are contained in the rendering pipe-line. Low-order rendering is of interest, when working with microphone arrays containing only a few sensors, or for reducing the bandwidth for signal transmission. Magnitude Least Squares rendering became the de facto standard for this, which discards high-frequency interaural phase information in favor of reducing magnitude errors. Building upon this idea, we suggest Masked Magnitude Least Squares, which optimized the Ambisonics coefficients with a neural network and employs a spatio-spectral weighting mask to control the accuracy of the magnitude reconstruction. In the tested case, the weighting mask helped to maintain high-frequency notches in the low-order HRTFs and improved the modeled median plane localization performance in comparison to MagLS, while only marginally affecting the overall accuracy of the magnitude reconstruction.

==> bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pics/Or.png}}]{Or Berebi}
received the B.Sc and M.Sc degrees in electrical and computer engineering in 2019 and 2022, respectively, from Ben-Gurion University of the Negev, Beer-Sheva, Israel, where he is currently working towards the Ph.D. degree. His current research interests focus on improving spatial audio perception for low order binaural reproduction.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pics/Zamir.jpg}}]{Zamir Ben-Hur}
is currently a research scientist at Meta Reality Labs Research, working on spatial audio technologies. He received the B.Sc. (summa cum laude), M.Sc. and Ph.D. degrees in electrical and computer engineering in 2015, 2017 and 2020 respectively, from Ben-Gurion University of the Negev, Beer-Sheva, Israel. His research interests include spatial audio signal processing for binaural reproduction with improved spatial perception.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pics/David.jpg}}]{David Lou Alon}
is a Research Scientist at Meta Reality Labs Research, investigating spatial audio technologies. He received his Ph.D. in electrical engineering from Ben Gurion University (Israel, 2017) in the field of spherical microphone array processing. His research areas include head-related transfer functions, spatial audio capture, binaural reproduction, and headphone equalization for VR and AR application.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pics/Boaz.jpg}}]{Boaz Rafaely}
(SM’01) received the B.Sc. degree (cum laude) in electrical engineering from Ben-Gurion University, Beer-Sheva, Israel, in 1986; the M.Sc. degree in biomedical engineering from Tel-Aviv University, Israel, in 1994; and the Ph.D. degree from the Institute of Sound and Vibration Research (ISVR), Southampton University, U.K., in 1997. 

At the ISVR, he was appointed Lecturer in 1997 and Senior Lecturer in 2001, working on active control of sound and acoustic signal processing. In 2002, he spent six months as a Visiting Scientist at the Sensory Communication Group, Research Laboratory of Electronics, Massachusetts Institute of Technology (MIT), Cambridge, investigating speech enhancement for hearing aids. He then joined the Department of Electrical and Computer Engineering at Ben-Gurion University as a Senior Lecturer in 2003, and appointed Associate Professor in 2010, and Professor in 2013. He is currently heading the acoustics laboratory, investigating methods for audio signal processing and spatial audio. During 2010-2014 he has served as an associate editor for IEEE Transactions on Audio, Speech and Language Processing, and during 2013-2018 as a member of the IEEE Audio and Acoustic Signal Processing Technical Committee. He also served as an associate editor for IEEE Signal Processing Letters during 2015-2019, IET Signal Processing during 2016-2019, and currently for Acta Acustica. During 2013-2016 he has served as the chair of the Israeli Acoustical Association, and is currently chairing the Technical Committee on Audio Signal Processing in the European Acoustical Association. 

Prof. Rafaely was awarded the British Council’s Clore Foundation Scholarship.
\end{IEEEbiography}
